On the Parameterized Complexity of Odd Coloring

A proper vertex coloring of a connected graph $G$ is called an odd coloring if, for every vertex $v$ in $G$, there exists a color that appears odd number of times in the open neighborhood of $v$. The minimum number of colors required to obtain an odd coloring of $G$ is called the \emph{odd chromatic number} of $G$, denoted by $\chi_{o}(G)$. Determining $\chi_o(G)$ known to be ${\sf NP}$-hard. Given a graph $G$ and an integer $k$, the \odc{} problem is to decide whether $\chi_o(G)$ is at most $k$. In this paper, we study the parameterized complexity of the problem, particularly with respect to structural graph parameters. We obtain the following results: \begin{itemize} \item We prove that the problem admits a polynomial kernel when parameterized by the distance to clique. \item We show that the problem cannot have a polynomial kernel when parameterized by the vertex cover number unless ${\sf NP} \subseteq {\sf Co {\text -} NP/poly}$. \item We show that the problem is fixed-parameter tractable when parameterized by distance to cluster, distance to co-cluster, or neighborhood diversity. \item We show that the problem is ${\sf W[1]}$-hard parameterized by clique-width. \end{itemize} Finally, we study the complexity of the problem on restricted graph classes. We show that it can be solved in polynomial time on cographs and split graphs but remains NP-complete on certain subclasses of bipartite graphs.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclu}
In this paper, we initiate the study of \odc~from the parameterzied complexity perspective. Similar to \textsc{Graph Coloring}, it is possible to formulate \odc{}~in MSO$_2$ with an additional constraint  , the problem becomes FPT parameterized by tree-width. \todo[]{let us remove the conlusion and add some open questions in the introduction itself towards the end. }

==> d2cluster-new.tex <==
\section{Distance to cluster new}

Let $f:X\rightarrow \{t'\}$ be a coloring of the vertices of $X$ where $t'\leq t$. Let $g:X\rightarrow \{t''\}$ where $t''\leq 2t$ be the color that acts as an odd color for the vertices of $X$. Let the colors used $f(X)\cup g(X)$ be $\{1, 2, \dots, t^*\}$. 
%$t^*$ denote the number of colors in $f(X)\cup g(X)$. 

Let $C_1, C_2, \dots, C_{\ell}$ be the maximal cliques in $G-X$. 
For each clique $C_{i}$ in $G-X$, let the vertices of $C_i$ 
be $\{v_{1, i}, v_{2,i}, \dots, v_{n_i, i}\}$ where $n_i=|C_i|$. 
We design a dynamic programming based algorithm to find the number of colors outside $[t^*]$ 
%besides the colors used for coloring the vertices of $X$ and the odd colors for the vertices of $X$, 
that are required to obtain an odd  coloring $h$ of $G$ such that $h|_X=f$ and the odd color of each vertex $v\in X$ is $g(v)$ that is $|h^{-1}(g(v)) \cap N(v)|$ is odd. 
%the vertices of $X$ are colored u. 
We define an entry $d[v_{i,j}, c, P, S, \widehat{S}, q]$ that defines the existence of a coloring $h:S\cup \{v_{1, 1, }, \dots, v_{i,j}\}\rightarrow [t^*+q]$ such that 
%coloring in $S\cup \{v_{1, 1, }, \dots, v_{i,j}\}$ such that 
\begin{itemize}
    \item each vertex in $C_1\cup C_2 \cup  \dots\cup C_{j-1}$ has an odd color, 
    \item each vertex in  $\{v_{1, j, }, \dots, v_{i,j}\}$ has an odd color,  \todo[]{I donot know how to write this}
    \item for each vertex $v\in X$, the parity of the number of neighbors of $v$ assigned the color $g(v)$ is $P(v)$, 
    \item $S\subseteq h(\{v_{1, j}, \dots, v_{i, j}\})\cap [t^*]$, i.e., the set of colors 
    %$S\subseteq [t^*]$ are 
    from $[t^*]$ used for the vertices $\{v_{1, j}, \dots, v_{i, j}\} $, 
    \item $\widehat{S}\subseteq h(\{v_{1, j}, \dots, v_{n_j, j}\})\cap [t^*]$, i.e., the set of colors 
    %$\widehat{S}\subseteq [t^*]$ 
    that will be used for the vertices $\{v_{1, j}, \dots, v_{i, j}\} $, 
    \item the number of vertices from $C_j$ that are assigned colors outside $[t^*]$ is at most $q$. and 
    \item there exists a clique $C_{w}$ where $w\in [j]$ such that 
    $h(C_w)\cap [t^*+1, t^*+q]=[t^*+1, t^*+q]$ 
    %such that $[t^*+1, t^*+q]\subseteq h(C_w)$ 
    and for every other clique $C_{w'}$ where $w'\in [j]\setminus \{w\}$ we have $h(C_w)\cap [t^*+1, t^*+q]\subseteq [t^*+1, t^*+q]$. 
    
\end{itemize}


\noindent
\textbf{Base case:} We set the entry $d[v_{1,1}, c, P, S, \widehat{S}, q]$ to {\sf true} if and only if the following conditions hold. 
\begin{itemize}
    \item $||$
\end{itemize}




%stores the minimum number of new colors required 

==> distance-clique.tex <==
\section{Distance to Clique}\label{gc-dc}

\begin{theorem}
	\odc{} admits a polynomial kernel when parameterized by the distance to clique.
\end{theorem}


\begin{proof}
	Let $(G,X, d, k)$ be an instance of \odc{}, where
	$X \subseteq V(G)$ of size $d$ such that $C=V(G) \setminus X$ is a clique of size $n-d$. 
	We assume that $k \geq |C|$, otherwise, the given instance is a trivial no instance, as we need $|C|$ colors to properly color the clique.  We assume that $|C| > d^2+1$, otherwise we trivially get a kernel of size at most $d^2+d+1$. Let $C_N=\{v \in C~|~ N(v) \cap X  =\emptyset\}$. If $|C_N| \geq d$, then the given instance is a yes instance and we get a trivial kernel. Therefore, we assume that $|C_N|<d$. 
	We now partition the vertices of $X$ based on their degree in the clique $C$. Let $X_{\ell}= \{x \in X : |N(x) \cap C| \leq d-1\}$, $X_{m}= \{x \in X : d \leq |N(x) \cap C| \leq n-2d-1\}$ and $X_h= \{x \in X : |N(x) \cap C| \geq n-2d\}$. 
	
	\begin{Reduction}
		Delete the vertices of $X_{m}$ from $G$ and the new instance is $(G-{X_{m}}, X \setminus X_m, d-|X_m|, k)$.
	\end{Reduction}
	\begin{lemma}
		Reduction Rule~1 is safe.
	\end{lemma}
	\begin{proof}
		\emph{Forward direction.} 
  Let $f$ be a $k$-odd coloring of $G$. We define a $k$-coloring 
  $g$ of $G - X_m$  as follows. 
  $g(v)=f(v)$ if $v \in X_h \cup C$. As each $v \in X_{\ell}$ has at most $d-1$ neighbors in $C$ and $|C|>d^{2}+1$, we color the vertices of $X_{\ell}$  with distinct colors in $g$.  
	
		Clearly $g$ is  a proper $k$-coloring of $G -X_m$. Consider a vertex $v \in X_h$, as $v$ has at least $d$ neighbors in $C$ at least one color in $f(N(v))$ appears exactly once in the neighborhood of $v$, and $v$ satifies odd coloring property. Consider a vertex $v \in C$, as $|C|>d^2+1$, $v$ satifies odd coloring property. 
		
		Finally consider a vertex $v \in X_{\ell}$. If odd color of $v$ in $f$ comes from outside $X_{\ell}$ then the same color is also an odd color in $g$.   If odd color of $v$ in $f$ comes from inside $X_{\ell}$
		then $v$ satifies odd coloring property as we have colored $X_{\ell}$ with distinct colors in $g$. Therefore $g$ is a odd coloring of $G -X_m$.
		
		\emph{Reverse direction.}
		Let $g$ be a $k$-odd coloring of $G -X_m$.
		We define a $k$-coloring of $G$ as follows. $f(v)=g(v)$ for each $v \in V(G-X_m)$.
		For each $v \in X_m$, we have  $|N(v) \cap C| \leq n-2d-1$, hence, we can color $X_m$ with $|X_m|$ many distinct colors (which are different from the colors used in $X_\ell \cup X_h)$  in $f$. As  $|N(v) \cap C| \geq d$, at least one color of $C$ appears exactly once in $N(v)$ for each $v \in X_m$. Therefore $f$ is a odd-coloring of $G$. 
	\end{proof}
	
	We assume that $X_h\neq \emptyset$, otherwise, using the above reduction rule and the property of $X_{\ell}$, we trivially get a kernel of size at most $d(d-1)+d$.  
	
	Let $D_h=\bigcap\limits_{x \in X_h}(N(x) \cap C)$ and $D_{\ell}=\bigcup\limits_{x \in X_{\ell}}(N(x) \cap C)$. It is easy to see that $|D_{\ell}| \leq d(d-1)$. Let $C_1=D_h \setminus D_{\ell}$. 
	
	
	\begin{lemma}~\label{lem-size}
		The size of $D_h$ is at least $n-(|X_h|+1)d$.
	\end{lemma}
	\begin{proof}
		As each vertex of $X_h$ has at least $n-2d$ neighbors in $C$, the
		number of edges $|E[X_h,C]|$ between $X_h$ and $C$ is at least $|X_h|(n-2d)$. 
		Suppose $|D_h|\leq n-(|X_h|+1)d-1$ then the number of edges $|E[X_h,D_h]|$ between $X_h$ and $D_h$ is at most  $|X_h|(n-(|X_h|+1)d-1)$. As each vertex of $C \setminus D_h$ can only have at most $|X_h|-1$ neighbors in $X_h$,  the number of edges $|E[X_h,C\setminus D_h]|$ between $X_h$ and $C \setminus D_h$ is at most $(|X_h|-1)(|X_h|d+1)$. Hence we have

	\begin{equation*}
	\begin{aligned}
		|E[X_h,C]| \leq {} & |E[X_h,D_h]|+ |E[X_h,C\setminus D_h]| \\
	& \leq  |X_h|(n-(|X_h|+1)d-1)+(|X_h|-1)(|X_h|d+1) \\
	& =|X_h|(n-2d)-1
	\end{aligned}
	\end{equation*}
	which is contradiction to the fact that $|E[X_h,C]| \geq |X_h|(n-2d)$.
	\end{proof}
	
    Therefore, we have $D_h \geq n-(|X_h|+1)d$.
    Hence $|C_1| \geq n-(|X_h|+1)d -d(d-1) \geq n-2d^2$. Let $C_2 \subseteq C_1$ be a set of $d+1$ arbitrary vertices. Let $C'=C_1 \setminus C_2$.

	\begin{Reduction}
		 Delete the vertices of $C'$ from $G$ and decrease $k$ by $|C'|$. The new instance is $(G \setminus C', X \setminus X_m, d-|X_m|, k-|C'|)$.
	\end{Reduction}
	\begin{lemma}
	Reduction Rule~2 is safe.
\end{lemma}
	\begin{proof}
		 \emph{Reverese direction.}
		 If $g$ is a $k-|C'|$ odd coloring of $G \setminus C'$ then we can get a $k$-odd coloring $f$ of $G$ from $g$ by coloring $C'$ with $|C'|$ many new distinct colors. 
		 
		 
		For the other direction, let $f$ be a $k$-odd coloring of $G$. We assume that $f(X_{\ell} )\cap f(C') = \emptyset$. If not, we recolor the vertices of $X_{\ell}$ with  $|X_{\ell}|$ many distinct colors from $f(C_2)$. 
		Observe that $N(C')=X_h \cup (C\setminus C')$, that is, in the coloring $f$ of $G$ each vertex of $C'$ receives a color different from each color in $X_{\ell} \cup X_h\cup (C\setminus C')$.  Therefore $f$ restricted to $G \setminus C'$ is a $(k-|C'|)$-proper coloring. We now argue that $f$ is also an odd coloring of $G \setminus C'$. 	Consider a vertex $v \in V(G \setminus C')$, if $v \in X_\ell$ then the odd color of $v$ in $G \setminus C'$ is same as the odd color of $v$ in $G$. If $v \in (X_h \cup (C \setminus C'))$, then as $C_2$ has $d+1$ vertices and at least one of the vertex color $c$ of $C_2$ is not used in $X_\ell \cup X_h$ by the coloring $f$. Hence, the color $c$ acts as a odd color for the vertex $v$. 
	\end{proof}
	
	It is easy to see that both reduction rules are applicable in polynomial time. Next, we show that the size of the reduced instance is at most $d^2+d$.
	
	\begin{lemma}
		Let $(G,X,d,k)$ be an instance of \odc{} obtained after applying the above reduction rules. If it is a yes instance then $|V(G)|\leq 3d^2+1$. 
	\end{lemma}
	\begin{proof}
			 
			We know that the size of $C'$ is at least $n-2d^2-d-1$. Therefore the number of vertices in $X_h \cup X_{\ell}\cup D_{\ell} \cup (C\setminus C')$ is at most $d+d(d-1)+(2d^2+1)$, which is $3d^2+1$.  
	\end{proof}
\vspace*{-0.5cm}	
\end{proof}


==> interval-new.tex <==
\section{Interval Graphs New}
Let $G$ be an interval graph and $\mathcal{I}$ be an \emph{interval representation} of $G$, i.e., 
there is
a mapping from $V(G)$ to closed intervals on the real line such that for any
two vertices $u$ and $v$, $uv \in E(G)$ if and only if $I_u \cap I_v \neq \emptyset$.
For any interval
graph, there exists an interval representation with all endpoints distinct. Such
a representation is called a \emph{distinguishing interval representation} and it can be computed starting from an
arbitrary interval representation of the graph. 
Interval graphs can be recognized in linear time and an interval representation can be obtained in linear time \cite{booth1976testing}.
 Let $l(I_u)$ and $r(I_u)$ denote the left and right end points of the interval corresponding
to the vertex $u$ respectively. We say that an interval $I \in \mathcal{I}$ is \emph{rightmost interval} if $r(J) \leq r(I)$ for all $J \in \mathcal{I}$.


\begin{theorem}\label{thm:inter}
    If $G$ is an interval graph, then $\omega(G)\leq \chi_o(G)\leq \omega(G)+1$. 
\end{theorem}

\begin{proof}
Let $G$ be an interval graph and $\mathcal{I}=\{I_{v_1},\ldots,I_{v_n}\}$ be an \emph{interval representation} of $G$.
Let $\mathcal{F}\subseteq \mathcal{I}$ which is constructed recursively as follows.
We select an interval $I_v \in \mathcal{I}$ such that $r(I_v) \leq r(I_u)$ for every $I_u \in \mathcal{I}$. Suppose $I_{v_1}, \ldots, I_{v_j}$ be the intervals selected to be part of $\mathcal{F}$. Next, we pick an interval $I_{v_{j+1}}$ such that $I_{v_{j+1}} \cap I_{v_j} \neq \emptyset$ and $r(I_{v_{j+1}})\geq r(I_{v_t})$ for every interval $I_t$ having $I_{v_{t}} \cap I_{v_j} \neq \emptyset$.  It is easy to see that the graph $G_{\mathcal{F}}$ induced by the intervals present in $\mathcal{F}=\{I_{v_1},\ldots,I_{v_r}\}$ is a path $P$ with vertices $\{v_1,\ldots,v_r\}$.

\begin{observation}\label{ob-interval-1}
For every interval $I_v \in \mathcal{I}$, there exists an interval $I_u \in \mathcal{F}$ such that $I_v \cap I_u \neq \emptyset$.
\end{observation}



\begin{observation}\label{ob-interval-2}
Let $I_v \in \mathcal{I}\setminus \mathcal{F}$ be an interval corresponding to the vertex $v$.  Then $v$ has at most two neighbors in $P$, that is $|N(v)\cap V(P)| \leq 3$. 
\end{observation}



\medskip
{\bf Phase~I.} 
In this phase we only color the vertices of path $P$. Let $f:V(P) \rightarrow \{1,2,3\}$
such that $f(v_i)=1$, if $i \equiv 1(\mod 3)$, $f(v_i)=2$, if $i \equiv 2(\mod 3)$ and $f(v_i)=3$, if $i \equiv 0(\mod 3)$.

By using observations~\ref{ob-interval-1} and \ref{ob-interval-2}, we can see that the partial coloring $f$ of $G$ is an odd coloring. That is, for every vertex $v$ in $G$, one of the colors form the set $\{1,2,3\}$ appears odd number of times in $N(v)$ in the coloring $f$. Notice that for every vertex $v_i \in V(P)$, two colors from the set $\{1,2,3\}$ appears exactly once in $N(v_i)$ in the coloring $f$. For every vertex $v_i\in V(P) \setminus \{v_1,v_r\}$, we fix $f(v_{i+1})$ as its odd color and release the color $f(v_{i-1})$, which is again used in the second phase. For vertex $v_1$, we fix $f(v_{2})$ as its odd color and For vertex $v_r$, we fix $f(v_{r-1})$ as its odd color.







\medskip
{\bf Phase~II.} 
We extend the partial coloring $f$ of $G$  to a total coloring $g$ of $G$ such that $g|_{V(P)}=f$. 

For every uncolored vertex $v$, we assign a list $L(v)$ of colors based on the following two cases.
%$L(v)=\{4,5,\ldots,k+1,f(v_{}$
%Let $v$ be an uncolored vertex with its corresponding interval $I_v$. We color $v$ based on the following two cases.

\medskip
{\bf Case~1.} $|N(v)\cap V(P)|=1$

Let $N(v)\cap V(P)=\{v_q\}$.
Then $L(v)=\{4,5,\ldots,k+1,f(v_{q-1})\}$

\medskip
{\bf Case~2.} $|N(v)\cap V(P)|=2$

Let $N(v)\cap V(P)=\{v_q,v_{q+1}\}$.
Then $L(v)=\{4,5,\ldots,k+1,f(v_{q-1})\}$


\medskip
{\bf Case~3.} $|N(v)\cap V(P)|=3$

Let $N(v)\cap V(P)=\{v_q,v_{q+1},v_{q+2}\}$.
Then $L(v)=\{4,5,\ldots,k+1\}$

It is easy to see that size of the largest clique in $G'=G[V(G) \setminus V(P)]$ is at most $k-1$ and $|L(v)|\geq k-2$. 
 Let $\{u_1,\ldots,u_{t}\}$ are the  vertices of $G'$, which are ordered as per the left ends point of their corresponding intervals. That is $u_i$ appears before $u_j$ if and only if $l(I_{u_i}) \leq l(I_{u_j})$. We color them greedily as per the above order as follows.
  $g(u_i)=\min \{L(u_i) \setminus T_i\}$, where $T_i$ denotes the set of colors used sofar in $N(u_i)$ in $G$. It is easy to see that $g$ is an odd coloring of $G$. 
\end{proof}

==> interval.tex <==
\section{Interval Graphs}\label{sec:int}


Let $G$ be an interval graph and $\mathcal{I}$ be an interval graph representation of $G$. 
We denote $L(I)$ and $R(I)$ to denote the left end point and the right end point of the interval $I$. Without loss of generality, we assume two intervals do not have the same end point (either left or right). We denote the maximum clique size of a graph $G$ by $\omega(G)$. 
%that the left and the right endpoints of the intervals 




\begin{theorem}\label{thm:inter}
    Let $G$ be an interval graph. Then $\omega(G)\leq \chi_o(G)\leq \omega(G)+1$. 
\end{theorem}

\begin{proof}
Let $k=\omega(G)$ and $\mathcal{I}$ be an interval graph representation of $G$. 
It is known that for any interval graph $G$, $\chi(G)=k$. 
%can be properly colored using $\omega(G)$ colors and that . 
Since odd-coloring is also a proper coloring, we have that $k \leq \chi_o(G)$. We now design an algorithm to obtain an odd coloring $g:\mathcal{I}\rightarrow [k+1]$ of $G$. We accomplish this in two phases. 
%using 
%$\omega(G)+1$ colors. 
%show the upper bound.  
%    We give a coloring $g:\mathcal{I}\rightarrow [k+1]$ in two phases. 
In the first phase we assign colors to some intervals to ensure that every interval in $\mathcal{I}$ has an odd color. 
    In the second phase, 
    we color the remaining uncolored intervals of $\mathcal{I}$. 

    
    Then we argue that $g$ is an odd coloring. 
    %Without loss of generality, we assume that the endpoints of any two intervals are distinct. 

    \medskip
    \noindent
    \textbf{Initial phase:} We pick the interval $I_1$ that has the least right end point and assign the color $1$. Then we pick the interval $I_2\in N(I_1)$ that has the rightmost end point among the neighbors of $I_1$ and assign $g(I_2)=2$. 
    For each $i\geq 3$, 
    we pick the interval $I_i$ that is adjacent to $I_{i-1}$ 
    and whose right end point is the largest. 
    Then assign $g(I_i)=\{1, 2, 3\}\setminus \{g(I_{i-1}), g(I_{i-2})\}$. Let $I_r$ be the interval that is colored the last in this process. 
    It is easy to see that the graph induced by the intervals $I_1, I_2, \dots, I_r$ forms an induced path. 
    Moreover, 
   the partial coloring is proper with the vertices assigned colors 1, 2 and 3 in an alternative fashion. 
\todo{you are interchangeably using a vertex $v$ with its interval $I_v$. We need color the vertices not the intervals. Because $g$ is a function with domain $V(G)$. }


  \begin{observation}\label{obs:ini-int}
      Each interval has an odd color from $\{1, 2, 3\}$. 
  \end{observation}  
  \todo{proof is not clear}
  \begin{proof}
      For each interval $I\in \mathcal{I}$, we have that $|N[I]\cap \{I_1, I_2, \dots, I_r\}|\geq 1$. 
      %Each vertex is adjacent to at least one colored vertex from $I_1, I_2, \dots, I_r$. Further, 
      Further because of our construction, $|g^{-1}(c)\cap N[I]|\leq 1$, for each $c\in\{1, 2, 3\}$. 
      For each interval $I\in \mathcal{I}\setminus \{I_1\}$, 
      we designate 
      %assign the $c$ as the odd color where 
      the color of the colored neighbor of $I$ with the smallest left end point as the odd color of $I$. 
%      is colored with $c$. 
For the interval $I_1$, we designate $g(I_2)$ as its odd color. 
      %where $c$ is the
      %a vertex is not adjacent to two vertices assigned the same color. 
      \qed
  \end{proof}

    Let $D$ denote the set of colored intervals from the initial phase. 
    %be $D$. 
    Consider the interval graph representation on 
    $\mathcal{I}\setminus D$. 
    %graph $G[V\setminus D]$. 
    We ask the following question: what is the size of a maximum clique in 
    $\mathcal{I}\setminus D$? Since each interval in $\mathcal{I}\setminus D$ intersects with at least one interval and at most two intervals in $D$, 
    the maximum sized clique in $\mathcal{I}\setminus D$ is either $k-2$ or $k-1$. 
    % If the size of a maximum sized clique in $\mathcal{I}\setminus D$ is $k-2$, then any proper coloring of $\mathcal{I}\setminus D$ together with $D$ 
    % is also an odd coloring of $\mathcal{I}$ using 
    % $k+1$ colors. 
    %with respect to $C$. 
    %Further, any interval in 
    %$G[V\setminus D]$? 
    \todo{More formal writing is needed.} 
    
    
    
    % Let $C$ be a maximum sized clique in $G[V\setminus D]$. Notice that $k-2 \leq |C|\leq k-1$. 
    % If $|C|=k-2$, then any proper coloring of $C$ is also an odd coloring with respect to $C$. 
    % %Any proper coloring of $C$ requires $k-2$ colors. 
    
    
    \begin{theorem}\label{thm:chor-inter}
        Chordal graphs that have a clique-tree which is a path are called interval graphs. 
    \end{theorem}
    %Suppose that the size of a maximum sized clique in $\mathcal{I}\setminus D$ is $k-1$. 
    Since $\mathcal{I}$ is an interval graph, from Theorem \ref{thm:chor-inter} there is a clique-tree decomposition $\mathcal{P}=(X,v_i)$
    of $\mathcal{I}\setminus D$ that is a path. Let the nodes of such a path be $v_1, v_2, \dots, v_{\ell}$.  
    %that corresponds to the interval representation of $G$. 
    We consider the nodes of $\mathcal{P}$ in order and color the vertices of $\mathcal{I}\setminus D$. 
    If the size of a maximum sized clique in $\mathcal{I}\setminus D$ is $k-2$, then any proper coloring of $\mathcal{I}\setminus D$ together with $D$ 
    is also an odd coloring of $\mathcal{I}$ using 
    $k+1$ colors. 
    
    Suppose that the size of a maximum sized clique in $\mathcal{I}\setminus D$ is $k-1$. Let $v_i$ be the node under consideration and $X(v_i)=C_i\subseteq \mathcal{I}\setminus D$. 
    Some of the vertices of $C_i$ may be colored by  the maximal cliques that appear before $C_i$. 
    Let $I_j\in D$ be the interval, 
    %assigned the color (say 2), 
    that together with $C_i$ forms a clique of size $k$ in $\mathcal{I}$. 
    %Let $I_{i-1}, I_{i+1}\in D$ be the set of colored neighbors adjacent to $I_i$,
    %and appear to the left and right of $I$. 
    %Let Notice that $g(I_p)=1$ and $g(I_n)=3$. 
    Recall that either the intervals $I_{j-1}$ and $I_{j+1}$ (if they exist) do not intersect with every vertex of $C_i$, 
    %does not belong to the clique of size $k$ in $\mathcal{I}$, 
    otherwise there is a clique of size greater than $k$. 
    %|C_i|=k-2$. 
    
    
    % We consider the maximal cliques in the clique-tree decomposition in order from root to the leaf. 
    % Let $C$ be the maximal clique under consideration. Some of the vertices of $C$ may be colored by  the maximal cliques that appear before $C$.  
    % Let $I_i\in D$ be the interval, 
    % that together with $C$ forms a clique of size $k$ in $G$. 
    % Recall that $I_{i-1}, I_{i+1}$ does not belong to the clique of size $k$ in $G$, otherwise $|C|=k-2$.  
    We give a coloring for the intervals in $C_i$ based on the following cases. 




\begin{itemize}
    \item \textbf{Each interval in $C_i$ is adjacent only to $I_1$ and not adjacent to $I_{2}$. } 

    We assign the color 3 to one of the vertices and the remaining vertices with $[k+1]\setminus \{1, 2, 3\}$. 

    \item \textbf{Each interval in $C_i$ is  not adjacent to 
    %$I_j$ and $j\geq 2$. } 
    is not adjacent to any of $I_{i-1}$ and $I_{i+1}$. } 

    %Let $I\in D$ be the interval, assigned the color (say 2), that together with $C$ is a clique of size $k$. Let $I_p, I_n\in D$ be the set of colored neighbors adjacent to $I$,
    %and appear to the left and right of $I$. Notice that $g(I_p)=1$ and $g(I_n)=3$. 
    Without loss of generality, let $g(I_i)=2$. 
    We arbitrarily pick an uncolored  vertex in $C$ and assign the color 3. 
    %Since $I$ has the color 1 as the odd color, and none of  the vertices in $C$ are adjacent to $I_p$ and $I_n$, 
    %we could use the color 3 to one of the vertices in $C$. 
    The remaining uncolored vertices are assigned colors from $[k+1]\setminus \{1, 2, 3\}$.     %Therefore the colors $[k+1]\setminus \{1, 2\}$ can be assigned to $C$. 

   \item \textbf{There exists an interval $I'\in N(I_i)\cap C$ that is not adjacent to $I_{i+1}$. }
   %$C$ contains an interval that is not adjacent to $I_n$} 

    We arbitrarily pick an uncolored  vertex in $C$ and assign the color 3. 
    %Since $I$ has the color 1 as the odd color, and none of  the vertices in $C$ are adjacent to $I_p$ and $I_n$, 
    %we could use the color 3 to one of the vertices in $C$. 
    The remaining uncolored vertices are assigned colors from $[k+1]\setminus \{1, 2, 3\}$.     %Therefore the colors $[k+1]\setminus \{1, 2\}$ can be assigned to $C$. 

   % \item \textbf{Every interval in $C$ is adjacent to $I_n$ (resp. $I_p$)} 

    %Then $C$ is adjacent to both $I$ and $I_n$ (resp. $I_p$), and thus $|C|=k-2$. 

    
    
\end{itemize}




    Let $I_i\in D$ be the interval, 
    %assigned the color (say 2), 
    that together with $C$ forms a clique of size $k$ in $G$. 
    
    
    
    
    %We now  consider the interesting case when $|C|=k-1$.    
    Let $I_i\in D$ be the interval, 
    %assigned the color (say 2), 
    that together with $C$ forms a clique of size $k$ in $G$. 
    %Let $I_{i-1}, I_{i+1}\in D$ be the set of colored neighbors adjacent to $I_i$,
    %and appear to the left and right of $I$. 
    %Let Notice that $g(I_p)=1$ and $g(I_n)=3$. 
    Recall that $I_{i-1}, I_{i+1}$ does not belong to the clique of size $k$ in $G$, otherwise $|C|=k-2$.  
    %is adjacent to both $I$ and $I_n$ (resp. $I_p$), and thus $|C|=k-2$. If every interval in $C$ is adjacent to $I_n$ (resp. $I_p$) 
    %then $C$ is adjacent to both $I$ and $I_n$ (resp. $I_p$), and thus $|C|=k-2$. 

There is a clique tree that corresponds to the interval representation of $G$. Consider the maximal cliques in the clique tree decomposition in order. 
Let $C$ be the maximal clique under consideration. 
\todo{This paragraph is not clear. We need to define the terms clique tree etc.}
%We order the intervals of $V\setminus D$ from left to right based on the increasing order of their left endpoints. 
%From the above discussion, 
%If an interval is part of a clique $C$ of size $k-1$, we assign the colors accordingly. 
Some of the vertices of $C$ may be colored by  the maximal cliques that apppear before $C$. 
    We give a coloring for the vertices in $V\setminus D$ based on the following cases. 



\begin{itemize}
    \item \textbf{Each interval in $C$ is adjacent only to $I_1$ and is not adjacent to $I_{2}$. } 

    We assign the color 3 to one of the vertices and the remaining vertices with $[k+1]\setminus \{1, 2, 3\}$. 

    \item \textbf{Each interval in $C$ is adjacent only to $I_i$ and is not adjacent to any of $I_{i-1}$ and $I_{i+1}$. } 

    %Let $I\in D$ be the interval, assigned the color (say 2), that together with $C$ is a clique of size $k$. Let $I_p, I_n\in D$ be the set of colored neighbors adjacent to $I$,
    %and appear to the left and right of $I$. Notice that $g(I_p)=1$ and $g(I_n)=3$. 
    Without loss of generality, let $g(I_i)=2$. 
    We arbitrarily pick an uncolored  vertex in $C$ and assign the color 3. 
    %Since $I$ has the color 1 as the odd color, and none of  the vertices in $C$ are adjacent to $I_p$ and $I_n$, 
    %we could use the color 3 to one of the vertices in $C$. 
    The remaining uncolored vertices are assigned colors from $[k+1]\setminus \{1, 2, 3\}$.     %Therefore the colors $[k+1]\setminus \{1, 2\}$ can be assigned to $C$. 

   \item \textbf{There exists an interval $I'\in N(I_i)\cap C$ that is not adjacent to $I_{i+1}$. }
   %$C$ contains an interval that is not adjacent to $I_n$} 

    We arbitrarily pick an uncolored  vertex in $C$ and assign the color 3. 
    %Since $I$ has the color 1 as the odd color, and none of  the vertices in $C$ are adjacent to $I_p$ and $I_n$, 
    %we could use the color 3 to one of the vertices in $C$. 
    The remaining uncolored vertices are assigned colors from $[k+1]\setminus \{1, 2, 3\}$.     %Therefore the colors $[k+1]\setminus \{1, 2\}$ can be assigned to $C$. 

   % \item \textbf{Every interval in $C$ is adjacent to $I_n$ (resp. $I_p$)} 

    %Then $C$ is adjacent to both $I$ and $I_n$ (resp. $I_p$), and thus $|C|=k-2$. 

    
    
\end{itemize}
We order the intervals of $V\setminus D$ from left to right based on the increasing order of their left endpoints. 
From the above discussion, if an interval is part of a clique $C$ of size $k-1$, we assign the colors accordingly. 
%based on the cases we first try to color the vertices with the 
%    \begin{itemize}
%        \item Pick an interval $I_1$ and assign the color 
%    \end{itemize}
    \qed
\end{proof}

\subsection{New Proof}
Consider the intervals in $\mathcal{I}\setminus D$ according to their right endpoints and assign colors. 
Let $I\in \mathcal{I}\setminus D$ be the uncolored interval under consideration. We maintain the invariant that  
%Without loss of generality, we assume that 
(a) all the intervals in $\mathcal{I}\setminus D$ whose right 
%whose right 
endpoint is less than $R(I)$ are properly colored and 
(b) all these colored intervals including $D$ 
have an odd color. 


\begin{itemize}
    \item \textbf{Case: $I$ is adjacent to only one interval $I_i\in D$. }

    This implies that $I$ is contained in $I_i$. 
    The number of colored neighbors of $I$ in $\mathcal{I}\setminus D$ is at most $k-2$. 
    
    If there exists a color $c\in \{1, 2, 3\}$ such that none of its neighbors are assigned the , then assign the minimum color from $\{4, 5, \dots, k+1\}$ that is not assigned to any of its colored neighbors. 
    
    If there exists a colored neighbor $I'\in \mathcal{I}\setminus D$ of $I$ such that $I'$ is assigned a color from $\{1, 2, 3\}$, then assign the minimum color from $\{4, 5, \dots, k+1\}$ that is not assigned to any of its colored neighbors. 

    Otherwise for each color $c\in \{4, 5, \dots, k+1\}$, there exists a neighbor of $I$ that is assigned the colors $c$. 
    %from all the colored neighbors of $I$ in $\mathcal{I}\setminus D$ are assigned colors from 
    
    
    \item \textbf{Case: $I$ is intersecting with two intervals $I_i, I_{i+1}\in D$. }
\end{itemize}
\subsection{Proper interval graphs}
Let $I_1$ and $I_2$ be two intervals of $\mathcal{I}$. 
%in the interval graph representation of $G$. 
We say $I_2$ is \emph{contained} in $I_1$ if  $L(I_1)<L(I_2)<R(I_2)<R(I_1)$. We say $I_2$ is a \emph{left neighbor} of $I_1$ if  $L(I_2)<L(I_1)<R(I_2)<R(I_1)$. Similarly, we say $I_2$ is a \emph{right neighbor} of $I_1$ if $L(I_1)<L(I_2)<R(I_1)<R(I_2)$. 

Since proper interval graphs are a subclass of interval graphs, 
from Theorem \ref{thm:inter} we get that $\chi_o(G)\leq \omega(G)+1$, where $G$ is a proper interval graph. Now we characterize proper interval graphs that require $\omega(G)+1$ colors. 


\begin{lemma}\label{lem:properint}
    Let $G$ be a proper interval graph. Then, 
    $\chi_o(G)=\omega(G)+1$ if and only if there is a vertex that participates in two maximum disjoint cliques. 
\end{lemma}

\begin{proof}
Let $k=\omega(G)$. 
Since $G$ is an interval graph, each vertex $v$ has at most $2(k-1)$ neighbors. Moreover, there are at most $k-1$ left neighbors and at most $k-1$ right neighbors. Consider a vertex $v$ that participates in two maximum disjoint cliques. Then the number of left neighbors and the number of right neighbors of $v$ is equal to $k-1$. Thus the reverse direction follows. 

Let $\chi_o(G)=k+1$. We prove it by contradiction. 
Suppose that there is no vertex that participates in two maximum disjoint cliques. Let $v_1, v_2, \dots, v_n$ be an ordering of the intervals arranged according to their right end points. 
Let $f:V(G)\rightarrow k$ be a coloring defined as follows. 
Assign $f(v_1)=1$. For each $i\geq 2$, if $f(v_{i-1})=k$ then assign $f(v_i)=1$. Otherwise, assign $f(v_i)=f(v_{i-1})+1$. We argue that $f$ is an odd coloring of $G$. It is easy to see that the vertex $v_{i}$ is not adjacent to the vertices $v_{i-k}$ and $v_{i+k}$. Otherwise there is a clique of size $k+1$, which is a contradiction. As any color in $[k]$ repeats after every $k$ vertices according to $f$, we can infer that $f$ is a proper coloring. 
    Also because of the assumption that there is no interval that participates in two maximum disjoint cliques, the maximum number of neighbors that an interval is at most $2(k-1)-1$. Thus there is a color that appears in the neighborhood of every vertex exactly once and thus features as the odd color. 
   \qed
\end{proof}


\begin{theorem}\label{thm:proper}
    \oc~is polynomial time solvable on proper interval graphs. 
\end{theorem}
The proof of the above theorem follows from Theorem \ref{thm:inter} and Lemma \ref{lem:properint}. 

==> neighborhood-diversity.tex <==
\section{Neighborhood Diversity}

\begin{definition}[Neighborhood Diversity~\cite{lampis2012algorithmic}]\label{def:nd}
Let $G=(V,E)$ be a graph. 
Two vertices $u,v\in V(G)$ are said to have the \emph{same type} if and only if $N(u)\setminus \{v\}=N(v)\setminus \{u\}$. A graph $G$ has neighborhood diversity at most $t$ 
if there exists a  partition of $V(G)$ into at most $t$ sets  
$V_1, V_2, \dots, V_t$ 
such that all vertices in each set have same type. 
\end{definition}
Observe that each $V_i$   either forms a  clique or an independent set in $G$.
Also, for any two distinct types
$V_i$ and $ V_j$, 
either each vertex in $V_i$ is adjacent to each vertex in $V_j$,
or no vertex in $V_i$ is adjacent to any vertex in $V_j$. 
We call a set $V_i$ as a \emph{clique type} (resp, independent type) if 
$G[V_i]$ is a clique (resp, independent set). If a type $V_i$ contains exactly one vertex then we call it as independent type. It is known that a smallest sized partition of $V(G)$ into clique types and independent types can be found in polynomial time \cite{lampis2012algorithmic}. Hence, we assume that the types $V_1, V_2, \dots, V_t$ of the graph $G$ are given as input. 

\begin{theorem}\label{thm:nd}
\odc~is FPT when parameterized by neighborhood diversity. 
\end{theorem}

We present an overview of the algorithm. We first observe that all vertices in an independent type has the same odd color. Since a clique type has at least two vertices and that an odd coloring is a proper coloring, any proper coloring will fetch an odd color for the vertices in the clique type. Thus we focus on the vertices in the independent types. We guess the set of independent types that have the same odd color. The number of such odd color is at most $t$. Further we guess the existence of a color in each of the types along with its parity. Then we adopt a coloring strategy to partially color some vertices and ensure that every vertex in the independent types has an odd color. We then claim that it is sufficient to properly color the remaining uncolored vertices and this leads to an odd coloring. 


We first look at some observations. 
%Each type $V_i$ such that $|V_i|=1$ is considered as an independent type. Thus each clique type $V_j$ has at least two vertices. 

\begin{observation}\label{obs:nd1}
    Let $u$ and $v$  be two vertices in an independent type $V_i$. Then $c$ is an odd color of $u$ if and only if $c$ is an odd color of $v$. 
\end{observation}

%\begin{observation}\label{obs:nd1}
%    Each vertex in an independent type $V_i$ has the same odd color. 
%\end{observation}
\begin{proof}
    The proof of this follows from the definition of the types. 
    \qed
\end{proof}
\begin{observation}\label{obs:nd-2}
    %Consider a clique type $V_i$ with $|V_i|\geq 2$. 
    Let $u$ and $v$ be two vertices in a clique type $V_i$ 
    and $f:V(G)\rightarrow [k]$ be an odd coloring of $G$. 
    Then 
    %an odd color for 
    each vertex $w\in V_i\setminus \{v\}$ has $f(v)$ as its odd color 
    and 
    $v$ has $f(u)$ as its odd color.  
\end{observation}
\begin{proof}
    Each vertex in the clique-type $V_i$ 
    is assigned a color if $f$ 
    that is distinct from all its neighbors in $V(G)$. 
    %Since $|V_i|\geq 2$, 
    Thus the claim follows. 
%    The proof follows from the definition of the types. 
\qed
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:nd}]
We first guess the set of independent types such that 
vertices from these types have the same odd color. Let $\mathcal{T}_i\subseteq \{V_1, V_2, \dots, V_t\}$ be the set of independent types that have the odd color $c_i$. 
%Consider an independent type $V_i$. From Observation \ref{obs:nd1}, each vertex in $V_i$ has the same odd color. Let the odd color for the vertices in $V_i$ be $c_i$. 
%that appears odd time of times in its neighborhood. 
We guess the subset type $A_i\subseteq \{V_1, V_2, \dots, V_t\}$ such that 
%be the subset of types such 
there exists a vertex from each of the types in $A_i$ that is assigned the color $c_i$. 
Further, let $g_i:A_i\rightarrow \{o,e\}$ be a function that assigns a value from $\{o, e\}$ to each type in $A_i$ indicating whether the color $c_i$ is assigned to odd number of vertices or even number of vertices in the type. 
%appears odd number of types or not. 
That is, 
for each $V_{\ell}\in A_i$, we assign 
$g_i(V_{\ell})=e$, if the number of vertices from $V_{\ell}$ that are assigned the color $c_i$ is even, 
and $g_i(V_{\ell})=o$, otherwise. 
%whether the color $c_i$ appears odd or even number of times in $V_i$. 
%Notice that vertices in two independent types can have the same odd color. 
Since there are at most $t$ independent types, the number of partitions $\mathcal{T}_i$, for which we guessed $A_i$ and $g_i$ is $r\leq t$. 
Without loss of generality, let the set of odd colors be $\{1, 2, \dots, r\}$. 

%for each $\mathcal{T}_i$we had guessed the color $c_i$, 
%the number of colors $c_i$ 
%for which we guessed $c_i$, $A_i$ and $g_i$ is at most $t$. 
%We have a color $c_i$, a subset type $A_i$ and a function $g_i$ for each independent type $V_i$. 

\begin{claim}\label{cla:ind}
    Given $c_i$, $A_i$ and $g_i$ for each $\mathcal{T}_i$, 
    %color $c_i$, a subset type $A_i$ and a function $g_i$ for an independent type $V_i$, 
    we can partially color the vertices of $G$ such that each vertex in the type from 
    %each vertex in 
    $\mathcal{T}_i$ has $c_i$ as an odd color.  
\end{claim}
\begin{proof}
We apply the following coloring scheme for each type $V_j\in A_i$. 
%Consider a type $V_j\in A_i$. 
If $g_i(V_j)=e$, 
we arbitrarily choose two uncolored vertices from $V_j$ and assign the color $c_i$. Else we arbitrarily choose an uncolored vertex from $V_i$ and assign the color $c_i$. Notice that we will be able to choose vertices according to the above process, else the choice of $A_i$ and $g_i$ is invalid. 

From Observation \ref{obs:nd1}, each vertex in $V_j$ has the same odd color and it is $c_i$. 
%is the same. 
By the choice of $A_i$ and $g_i$, it so happens that the number of times the color $c_i$ appears in the neighborhood of each vertex in $V_j$ is odd. Thus each vertex in $V_j$ has an odd color. 
    \qed
\end{proof}

From Observation \ref{obs:nd-2}, it is clear that any proper coloring of $G$ ensures 
%a clique type $V_i$ ensures 
an odd color for each vertex in a clique type. 
Thus we shift our focus to extend the partial coloring of $G$ to the remaining vertices of $G$ such that each uncolored vertex is assigned a color such that no two adjacent vertices receive the same color. Since all vertices in the clique are assigned distinct colors in any odd coloring, according to our choices $A_i$ and $g_i$ we must have assigned a vertex the color $c_i$ or none of the vertices the color $c_i$. Now we move to the independent types. 
%a proper coloring of $G$. what remains is to properly color the remaining vertices of the graph. 
We say an independent type is \emph{partially colored} if there exists a vertex that is assigned a color in the above process. 
We first give a coloring process to color the uncolored vertices of a partially colored independent type $V_j$.  
%extend the coloring of a partially colored independent type 
%$V_j$. 
%We divide the coloring process based on whether there exists a color $c'$ is assigned to odd or not. 
Let $d_j$ denote the number of vertices from $V_j$ that are colored according to the above process. 
Depending upon the size of $V_j$, we have the following cases: 

\begin{itemize}
    
    \item $|V_i|$ is even. 
    \begin{itemize}
        \item \textbf{$d_i$ is even  and there is a color $c\in [r]$ 
        that is assigned to even number of vertices in $V_i$. }
        %$W_i^+\neq \emptyset$.  

        %No extra color is required for coloring the remaining vertices of $V_i$. 
        We assign the color $c$ to each uncolored vertex of $V_i$. Since $|V_i|-d_i$ is even, the number of vertices assigned the color $c$ in $V_i$ is still even. 
        %from $W_i^+$. 

    \item \textbf{$d_i$ is even and there is no color that is assigned to even number of vertices in $V_i$. }
    %$|W_i^+|=\emptyset$.  


This implies that the number of colors 
that are assigned to odd number of vertices in $V_i$ is even. 
We arbitrarily pick a color $c$ that is assigned to a vertex in $V_i$ and 
assign it to the remaining uncolored vertices of $V_i$. Since $|V_i|-d_i$ is even, the number of vertices assigned the color $c$ in $V_i$ is still odd. 

        \item \textbf{$d_i$ is odd.} 
        %and there is a color $c$ that is assigned to odd number of vertices. }

        If there is an extension of the precoloring to $V_i$ and $[r]$, since $|V_i|-d_j$ is odd,   
        there exists a color $c$ that is assigned to odd number of uncolored vertices in $V_i$. Suppose $c$ was assigned to odd number of vertices in the precoloring of $V_i$, then after the above coloring step, $c$ is assigned to even number of vertices in $V_i$, which contradicts the choice of $g_i(V_i)$ that $c_i$ should be assigned to odd number of colors. The same is true when we pick the color $c$ was assigned to even number of vertices in the precoloring. 

        Thus we need a new color outside $[r]$ to color the uncolored vertices of $V_i$. 
        
        %a color that is assigned to odd or even number of 
        %Each of the color $c$ that is assigned to odd number of vertices, can now be assigned to even number of vertices to maintain that requirement that $c$ is assigned to odd number of vertices in $V_i$. 
        %In addition, the same is true for the colors $c$ that is assigned to even number of vertices. 
        %Thus  we cannot extend the coloring using the colors assigned in the precoloring of $V_i$. 
        %One extra color is  needed.      
    \end{itemize}

    \item $|V_i|$ is odd. 
 \begin{itemize}
 
       \item \textbf{$d_i$ is odd and 
        and there is a color $c\in [r]$ that is assigned to even number of vertices in $V_i$. }
       %$|W_i^+|\neq \emptyset$.  

        %No extra color is required for coloring the remaining vertices of $V_i$. 
  
    
    We assign the color $c$ to each uncolored vertex of $V_i$. Since $|V_i|-d_i$ is even, the number of vertices assigned the color $c$ in $V_i$ is still even. 
        
 %       We assign the color $c$ to each uncolored vertex of $V_i$. 
        %from $W_i^+$. 

     \item \textbf{$d_i$ is odd and 
     and there is no color that is assigned to even number of vertices in $V_i$. }
     %$|W_i^+|= \emptyset$.  


This implies that the number of colors 
that are assigned to odd number of vertices in $V_i$ is odd. 
We arbitrarily pick a color $c$ that is assigned to a vertex in $V_i$ and 
assign it to the remaining uncolored vertices of $V_i$. Since $|V_i|-d_i$ is even, the number of vertices assigned the color $c$ in $V_i$ is still odd. 


%Then the number of colors assigned to odd number of vertices in $V_i$ is even. 
%$|W_i^-|$ is even. No extra color needed. 
%We arbitrarily pick a color that is assigned to a vertex in $V_i$ 
%$W_i^-$ 
%and assign it to the remaining uncolored vertices of $V_i$. 

    \item \textbf{$v_i$ is even. }
     %and $W_i^+\neq \emptyset$. 

      We need an new color outside $[r]$ to color the uncolored vertices of $V_i$, and the arguments are similar in nature to the case when $|V_i|$ is even and $v_i$ is odd. 
      %Same arguments as in the above case. %One extra color is required.   

 \end{itemize}
%\todo[]{The cases are similar in both the settings. Written it for our understanding. We should simplify later. }
 
 \end{itemize}
From the above coloring process, we have a precoloring of the vertices of $G$ using the colors from $[r]$. 
%Let the number of colors used in the precoloring of $G$ be $q$. 
We construct an auxiliary graph $G'$ from $G$ where $V(G')$ is the set of all uncolored vertices of $G$ and $E(G')=\{uv\in E(GH)\mid u,v\in V(G')\}$. 
Notice that the graph $G'$ may be disconnected.  
Since $G'$ is a subgraph of $G$, the neighborhood diversity fo $G'$ is at most $t$. 
%Let $D$ be a connected component $D$ of $G'$. 
%Notice that the neighborhood diversity of $D$ is at most $t$. \textcolor{red}{We may not have to say this explicitly} 
\begin{claim}\label{cla:gg'}
    There is an odd coloring of $(G, t)$ using $r+s$ colors satisfying the guess $A_i$ and $g_i$ for each $i\in r$, 
    if and only if there is a proper coloring of $(G', t)$ using $s$ colors.  
\end{claim}
The proof of the above theorem is trivial and hence we omit the proof. 
We use the following theorem from \cite{robert-g-nd} to obtain the chromatic number of $G'$ and thus obtain an odd coloring of $G$. 
\begin{theorem}[\cite{robert-g-nd}]\label{thm:graphcoloring-nd}
   The \textsc{Precoloring Extension} problem can be solved in time
$O(q^{2.5q+o(q)} \cdot n)$, where $q = 2^{2t}$, on graphs of neighborhood diversity at most $t$. 

%\textsc{Graph Coloring} can be solved in time $2^{2^{2k}}n^{O(1)}$ on graphs of neighborhood diversity $t$. 
\end{theorem}

This complete the proof. We now give the running time of the algorithm. 
%\paragraph{Running time:} 
Guessing the partition of independent types that receive the same odd color, 
$A_i$ and $g_i$ for each $i\in [r]$ 
can be done in time $t^t2^{O(t^2)}$. The precoloring extension of coloring (if exists) for an independent type can be done 
in polynomial time. The graph $G'$ can be constructed in polynomial time. Obtaining the chromatic number for $G'$ can be done in time $O(2^{O(t2^{2t})}\cdot n)$. 
Thus the overall running time is $2^{O(t2^{2t})}n^{O(1)}$. 
%Where does the color $c_i$ exclusively belong to and whether they appear in odd or even number of times. 
\qed    
\end{proof}

\begin{comment}
    \subsection{Old}
\medskip
\noindent
\textbf{Question 1:} Consider an independent type $V_i$. There is a color, say $c_i$,   that appears odd time of times in its neighborhood. Where does the color $c_i$ exclusively belong to and whether they appear in odd or even number of times. 


Let $A_i\subseteq \{V_1, V_2, \dots, V_t\}$ be the subset of type that exclusively has the color $c_i$. Also let $B_i:A_i\rightarrow \{+,-\}$ be a function that assigns each type in $A_i$ 
whether the color $c_i$ appears odd or even number of times in $V_i$. 
We assign $B_i(V_j)=+$ if the number of vertices from $V_j$ assigned the color $c_i$ is even. Otherwise $B_i(V_j)=1$. 

Assign the respective color to the subset $A_i$ and reduce $k$ by 1. Now all the vertices in independent types have odd colors in their neighborhood. The cliques have their odd color from within the clique. 

\medskip
\noindent
\textbf{Question 2:} Each independent type $V_i$ has some colors $W_i^-$ repeated odd number of times and some colors $W_i^+$ repeated even number of times. How to assign colors to $V_i$. 

    We design a partial coloring process as follows: 
    \begin{itemize}
        \item for each color $c\in W_i^-$, 
    pick an arbitrary uncolored vertex from $V_i$ and assign the color $c$. 
    \item for each color $c\in W_i^+$, 
    pick two arbitrary uncolored vertices from $V_i$ and assign the color $c$. 
    \end{itemize}



Let $\widehat{V_i}$ denote the number of vertices from $V_i$ assigned colors either from the coloring process described for question 1 or question 2. Depending upon the size of $V_i$, we have the following cases: 

\begin{itemize}
    \item $|V_i|=0$

    One extra color is needed. 
    \item $|V_i|$ is even. 
    \begin{itemize}
        \item $|\widehat{V_i}|$ is even  and $W_i^+\neq \emptyset$.  

        No extra color is required for coloring the remaining vertices of $V_i$. We can assign a color from $W_i^+$. 

    \item $|\widehat{V_i}|$ is even and $|W_i^+|=\emptyset$.  


Then $|W_i^-|$ is even. No extra color needed. Arbitrarily pick a color from $W_i^-$ and assign it to the remaining uncolored vertices of $V_i$. 

        \item $|\widehat{V_i}|$ is odd. 
        %and $W_i^+\neq \emptyset$. 


        One extra color is  needed. 
%         \begin{itemize}
%             \item $|W_i^-|$ is odd. 

%             Extra color required. 

%             \item $|W_i^-|$ is even. 

%              No extra color is required. 
              
%         \end{itemize}
%No extra color is required for coloring the remaining vertices of $V_i$. We can assign a color from $W_i^+$. 
        
%        \item $|\widehat{V_i}|$ is odd and $W_i^+= \emptyset$. 
        
%         This implies that $|W_i^-|$ is odd. 
%One extra color is required.         
    \end{itemize}

    \item $|V_i|$ is odd. 
 \begin{itemize}
     \item $|\widehat{V_i}|$ is even. 
     %and $W_i^+\neq \emptyset$. 

      One extra color is required.   

       \item $|\widehat{V_i}|$ is odd and $|W_i^+|\neq \emptyset$.  

        No extra color is required for coloring the remaining vertices of $V_i$. We can assign a color from $W_i^+$. 

             \item $|\widehat{V_i}|$ is odd and $|W_i^+|= \emptyset$.  

Then $|W_i^-|$ is even. No extra color needed. Arbitrarily pick a color from $W_i^-$ and assign it to the remaining uncolored vertices of $V_i$. 


 \end{itemize}
 
 
 \end{itemize}

        
%        No extra color is required for coloring the remaining vertices of $V_i$. We can assign a color from $W_i^+$. 



        
%    In this way each color from $W_i^-$ and $W_i^+$ is assigned to $V_i$. 
If the cases where an extra color is needed, a subset of such independent types could be assigned the same color. In addition, 
that extra color could be assigned to some of the clique types. Since the number of independent types is at most $t$, for each of the independent type $V_i$ we guess the set of types that receive the extra color that vertices in $V_i$ are assigned. This can be done in time $2^{t^2}$.  
%color that 

Let $G'$ be the graph obtained from $G$ by removing the colored vertices of $G$. The resultant graph has neighborhood diversity at most $t$, and each of the types is a clique type. We now use the graph coloring parameterized by neighborhood diversity parameter to obtain an FPT algorithm for odd coloring problem. 


\end{comment}


==> tw.tex <==
\section{Tree-width}

\begin{theorem}\label{thm:tw}
    $\chi_o(G)\leq 2{\sf tw}(G)+1$. 
\end{theorem}

\begin{proof}
At each bag $X_t$ in a nice tree decomposition, 
    \begin{itemize}
        \item the number of colors required for proper coloring of $X_t$ is ${\sf tw}(G)+1$. 
        \item at each introduce node $t$, where $X_t=X_{t'}\cup \{v\}$ and $t'$ is the child node of $t$, 

        we fix a color $c$ that appears in the neighborhood of $v$ as its odd color and ensure that $c$ appears exactly once $N(v)$. 

        \item we assign a minimum color that is not assigned to the neighbors of $v$ and also their respective odd colors. Since the number of such colors is $2{\sf tw}(G)$, we use a at most one new color for $v$. 
    \end{itemize}
    \qed
\end{proof}
